An STL-based Approach to Resilient Control for Cyber-Physical Systems

We present ResilienC, a framework for resilient control of Cyber-Physical Systems subject to STL-based requirements. ResilienC utilizes a recently developed formalism for specifying CPS resiliency in terms of sets of $(\mathit{rec},\mathit{dur})$ real-valued pairs, where $\mathit{rec}$ represents the system's capability to rapidly recover from a property violation (recoverability), and $\mathit{dur}$ is reflective of its ability to avoid violations post-recovery (durability). We define the resilient STL control problem as one of multi-objective optimization, where the recoverability and durability of the desired STL specification are maximized. When neither objective is prioritized over the other, the solution to the problem is a set of Pareto-optimal system trajectories. We present a precise solution method to the resilient STL control problem using a mixed-integer linear programming encoding and an a posteriori $\epsilon$-constraint approach for efficiently retrieving the complete set of optimally resilient solutions. In ResilienC, at each time-step, the optimal control action selected from the set of Pareto-optimal solutions by a Decision Maker strategy realizes a form of Model Predictive Control. We demonstrate the practical utility of the ResilienC framework on two significant case studies: autonomous vehicle lane keeping and deadline-driven, multi-region package delivery.

==> introduction.tex <==
\section{Introduction}

Resiliency is of fundamental importance in cyber-physical systems (CPSs), as in numerous application domains these systems are expected to fulfill safety- and mission-critical requirements even in the presence of internal faults or external disturbances. 
For instance, in a lane-keeping problem, a vehicle intends to stay in its driving lane. However, staying in the lane can be dangerous or even inadmissible when the vehicle is affected by external disturbances such as other vehicles approaching excessively close. In such cases, the vehicle might violate the lane-keeping requirement to avoid a collision. Nonetheless, it should resiliently re-satisfy the lane-keeping requirement as soon as possible, and subsequently, maintain in the lane as long as possible.

Researchers have been trying to understand and formulate resilience in CPS. Signal temporal logic (STL)~\cite{maler2004monitoring} is a formal specification language for real-valued signals and is often used for formulating temporal specifications. An STL-based resiliency specification (SRS) logic~\cite{chen2022stl} is used to formulate the resiliency of STL formulas as the joint satisfaction of recoverability and subsequent durability properties. Given an arbitrary STL formula $\varphi$, the SRS formula $\srs_{\Trec,\Tdur}(\varphi)=\neg \varphi\mathbf{U}_{[0,\Trec]}\mathbf{G}_{[0,\Tdur)}\varphi$ specifies the following properties: the ability to recover from a violation of $\varphi$ within a time bound $\Trec$ and the subsequent ability to maintain $\varphi$ for at least time $\Tdur$.  Given $\srs_{\Trec,\Tdur}(\varphi)$, a signal and a time, a quantitative $(\mathit{rec},\mathit{dur})$ pair can be computed to measure the resilience of $\varphi$. The $\mathit{rec}$ and $\mathit{dur}$ values respectively quantify how long before the time-bound $\Trec$ the satisfaction of $\varphi$ occurs and subsequently how long the satisfaction is maintained after another time-bound $\Tdur$.

Control of dynamic systems subject to STL specifications has been studied~\cite{raman2014model,rodionova2021time} with a variety of control objectives and constraints, however, the area of control frameworks that aims to maximize the resilience of STL specifications remains largely unexplored. We propose a resilient control framework, called \emph{\name}, that predicts the optimal trajectories of the control system that represent the best-case resilience of the STL specifications to which the system is subject, then implements one of the optimal control actions selected by a decision-maker (DM) in a model predictive control (MPC) scheme.

We define the \emph{\probname} problem as an optimization problem whose decision variables are the control actions of a discrete-time, linear dynamic system. It has two resiliency maximization objectives (i.e., recoverability and durability of an STL formula $\varphi$), namely, the cost functions are the $\mathit{rec}$ and $\mathit{dur}$ values of $\srs_{\Trec,\Tdur}(\varphi)$ with respect to the predicted system states at time 0.
In this multi-objective problem, we use a (non-Pareto) dominance relation for indicating two solutions are equally resilient and non-dominated, resulting in a set of \emph{non-dominated optimal solutions}.
To solve the \probname problem, we first encode it with mixed-integer linear programming (MILP) constraints and objectives, converting it to a multi-objective MILP problem.
% The objective is to find the optimal control actions that maximize both the recoverability and durability of the desired STL property with respect to the states of the control system. 
% The optimal solution of the optimization problem contains a set of non-dominated $(\mathit{rec},\mathit{dur})$ objective pairs in the sense that no pair dominates others in the set. 
Then, we design an a-posteriori method for efficiently computing the set of optimal solutions by solving multiple instances of single-objective MILP problems. We prove our solution method is correct and analyze its computation complexity.  
Moreover, we design DMs representing different preference criteria to select a single solution from the resulting set of optimal solutions. With the corresponding optimal control actions, we adopt an MPC scheme by iteratively solving the \probname problem at each time step and implementing the first control action.
See Figure~\ref{fig:overall} for an architectural overview of the \name framework.

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{img/overall.png}
	\caption{Architectural overview of \name.}
	\label{fig:overall}
\end{figure}

We perform an experimental evaluation of \name upon two case studies: lane keeping and deadline-driven multi-region package delivery. Our results clearly demonstrate the effectiveness of our solution method and the details behind each non-dominated optimal solution. Control systems under MPC control are evaluated to demonstrate the difference in DM preferences.

We conclude our contributions as follows.
\begin{itemize}
    \item We propose \name, a resilient control framework for dynamic systems under STL specifications. We define \probname as a multi-objective optimization problem that maximizes the recoverability and durability of the STL specifications and generates a set of non-dominated optimal solutions. We also propose various DM for selecting a single optimal solution thus the framework can implement control actions via an MPC scheme. 
    \item We propose a solution method for \probname problem. We design an algorithm that applies MILP encoding to the problem and uses an a-posteriori method to efficiently compute the set of optimal solutions by solving single-objective MILP problems. 
    \item We conduct experimental evaluation via two case studies and demonstrate optimal solutions that represent vastly different but equivalently resilient trajectories. The case studies also illustrate the preferences of DM in MPC control. 
\end{itemize}

In the remaining sections, Section~\ref{sec:background} introduces the background of STL and  STL-based resilience in CPS. Section~\ref{sec:prob_form} provides the definition of the \probname problem and its relations to other problems in literature.  Section~\ref{sec:solution_method} provides our solution method for the \name framework. Section~\ref{sec:mpc_dm} describes the MPC strategy and our DM design. Section~\ref{sec:casestudy} demonstrates two case studies. Section~\ref{sec:related} discusses literature of related work. Section~\ref{sec:conclusion} concludes our work.

==> tables/lk_dms.tex <==
\begin{table}[t]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
        DMs & recoverability (s) & durability (s) & $\#$ of $P_\epsilon$ \\ \midrule
Random & 0.11 & -2.04 & 1.45  \\ \midrule
Pro-recoverability & 0.2 & -2.1 & 1.28  \\ \midrule
Pro-durability & -0.1 & -1.9 & 1.45  \\ \midrule
Minimal distance & -0.1 & -1.9 & 1.45  \\ \midrule
Adaptive & 0.1 & -2.1 & 1.38  \\\bottomrule
\end{tabular}
\caption{Resilience of vehicle trajectory with different DMs and an MPC scheme in a lane-keeping problem.} 
\label{tab:lk_dms}
\end{table}
